Is It Safe to Uplift This Patch? An Empirical Study on Mozilla Firefox

In rapid release development processes, patches that fix critical issues, or implement high-value features are often promoted directly from the development channel to a stabilization channel, potentially skipping one or more stabilization channels. This practice is called patch uplift. Patch uplift is risky, because patches that are rushed through the stabilization phase can end up introducing regressions in the code. This paper examines patch uplift operations at Mozilla, with the aim to identify the characteristics of uplifted patches that introduce regressions. Through statistical and manual analyses, we quantitatively and qualitatively investigate the reasons behind patch uplift decisions and the characteristics of uplifted patches that introduced regressions. Additionally, we interviewed three Mozilla release managers to understand organizational factors that affect patch uplift decisions and outcomes. Results show that most patches are uplifted because of a wrong functionality or a crash. Uplifted patches that lead to faults tend to have larger patch size, and most of the faults are due to semantic or memory errors in the patches. Also, release managers are more inclined to accept patch uplift requests that concern certain specific components, and-or that are submitted by certain specific developers.

==> tex_files/case_study3.tex <==
\subsection*{RQ3: \RQthree}

\noindent
\emph{\textbf{Motivation.}}
According to the results of \textbf{RQ2}, there are statistically significant differences between the characteristics of uplifted patches that introduced regressions and those that were integrated successfully (\ie{} clean uplifts that did not induced faults). %issues which are allowed to uplifted and which are rejected, and differences between fault-prone uplifted issues and clean uplifted issues.
In this research question, we further explore the relationship between the fault-proneness of an uplifted patch and a series of development- and human-related factors. The answer to this question can raise the awareness of software release managers toward important factors that could explain why certain uplifted patches introduce regressions in the code; helping them improve the reliability of patch uplift operations. % development and review process, and the uplifting rules.

\noindent
\emph{\textbf{Approach.}}
Using the metrics described in Table~\ref{tab:all_metrics} (as independent variables), we select two machine learning algorithms (\emph{decision tree} and \emph{Multivariate Adaptive Regression Splines} (MARS)) to model the fault-proneness of uplifted patches. Decision tree is a classification approach widely used to explain or predict a binary result. We choose this algorithm because a decision tree model can clearly illustrate how the independent variables (\ie{} the metrics) affect the fault-proneness of an uplifted patch. In this paper, we use the R package \texttt{rpart} \cite{therneau1997introduction} to build decision trees. Because \texttt{rpart} can yield easily interpretable results, and the \texttt{rpart.plot} package allows us to customize the output of decision tree figures. Multivariate Adaptive Regression Splines (MARS) is a non-linear regression technique. Compared to linear regression models, the MARS algorithm does not stick to an assumption of linear relationship between the independent and dependent variables. And compared to other non-linear algorithms, such as Harrell Jr.'s \texttt{rms} models \cite{harrell2013regression}, MARS models can be automatically built. Thus, the models can avoid biases from modellers' experience. In practice, MARS models have been successfully applied in different fields, such as medical and economics domains~\cite{york2000common,osei2004exploring}. Bettenburg et al.~\cite{bettenburg2015towards} also observed that this algorithm can yield good prediction results for software engineering datasets. In this paper, we use the R package \texttt{earth} to build MARS models.

To deal with the collinearity among the independent variables, we perform the Variance Inflation Factor (VIF) analysis before feeding the variables into the models. As recommended by prior works, such as \cite{rogerson2010statistical}, we remove all variables with VIF values equal or larger than 5.

The fault-inducing uplifts only account for 8.8\%, 8.3\%, and 7.9\% in the Aurora, Beta, and Release channels, respectively. Previous work shows that the imbalance in the dataset can degrade the performance of the explanatory models~\cite{kamei2007effects}. To deal with this problem, we perform a combination of over- and under-sampling using the R \texttt{ovun.sample} package. Concretely, instances in the majority category (\ie{} clean uplifts) will be randomly deleted and the the minority category (\ie{} fault-inducing uplifts) will also be randomly boosted, until the number of the instances in both categories achieve the same level.

To help release managers improve their uplift strategy, we will report the most important metrics yielded by the models.

\begin{figure}[t]
\centering
\includegraphics[width = 0.7\linewidth]{images/tree.pdf}
\caption{Decision tree on Aurora channel's fault-proneness (nodes not shown are automatically pruned by the algorithm).}
\label{fig:tree_example}
\vspace{-15pt}
\end{figure} 

\begin{table}[t]
\centering\scriptsize
\caption{\label{tab:r2} {$R^2$} of the explanatory models}
	\begin{tabular}{l|lll}
	\toprule
	\textbf{Algorithm} & \textbf{Aurora} & \textbf{Beta} & \textbf{Release}\\
	\midrule
	Decision tree & 0.50 & 0.52 & 0.78 \\
	MARS & 0.31 & 0.33 & 0.87 \\
	\bottomrule
	\end{tabular}
\end{table}

\begin{table}[t]
\centering\scriptsize
\caption{\label{tab:rank_tree} {Decision trees' top three nodes to classify whether an uplifted patch is fault-inducing}}
	\begin{tabular}{l|lll}
	\toprule
	\textbf{Channel} & \textbf{Top node} & \textbf{Second node} & \textbf{Third node}\\
	\midrule
	Aurora & code churn & PageRank & test code churn\\
	\hline
	Beta & \multirow{3}{*}{code churn} & \multirow{2}{*}{code churn} & cyclomatic \\
	{} & {} & {} & PageRank \\ \cline{3-4}
	{} & {} & PageRank & owner sentiment \\
	\hline
	Release & \multirow{4}{*}{code churn} & \multirow{2}{*}{developer exp.} & \# of prior changes\\
	{} & {} & {} & comment words \\ \cline{3-4}
	{} & {} & \multirow{2}{*}{\# of functions} & PageRank \\
	{} & {} & {} & code churn \\
	\bottomrule
	\end{tabular}
\vspace{-10pt}
\end{table}

\begin{table}[t]
\centering\scriptsize
\caption{\label{tab:rank_mars} {MARS top five metrics to classify whether an uplifted patch is fault-inducing}}
	\begin{tabular}{r|lll}
	\toprule
	\textbf{Rank} & \textbf{Aurora} & \textbf{Beta} & \textbf{Release}\\
	\midrule
	1 & code churn & code churn & max. nesting \\
	2 & closeness & max. nesting & comment words \\
	3 & \# function & \# prior changes & closeness \\
	4 & release delta & developer exp. & PageRank \\
	5 & comment words & LOC & comment ratio \\
	\bottomrule
	\end{tabular}
	\vspace{-10pt}
\end{table}


\noindent
\emph{\textbf{Results.}} Table~\ref{tab:r2} shows the $R^2$ obtained for the two algorithms in each of the three release channels. The higher the $R^2$ value, the better the fitness of a model. Both algorithms can achieve a high $R^2$ on the data from the Release channel, but decision tree has a more stable performance across the three channels.

Figure~\ref{fig:tree_example} depicts the decision tree on the fault-proneness for the Aurora channel. Due to the page limit, we only show one decision figure in the paper. Other tree figures are available in our online repository.
Table \ref{tab:rank_tree} summarizes decision trees' top three nodes to classify whether an uplift patch can lead to faults. Each top node has two second nodes, which may have 1-2 third node(s). In the table, we use a line across the columns second node and third node to represent the relationship between the second nodes and third nodes. For example, the second node, code churn, in Beta has two third nodes: cyclomatic and PageRank.
We observed that code churn plays the most important role in all three channels. This result is expected, because large changes are more likely to contain faults and they are more difficult to review. Reviewers and release managers might omit faults contained in patches with large code churn values, letting these faults slip in the release version that is distributed to end users. In addition, PageRank values can also explain the fault-proneness of an uplift patch, across all the three channels. Because when we modify a class that is connected to many other classes, the risk of faults is increased by the complex dependencies. In \textbf{RQ2}, we did not observe a significant difference between the churn of test code for fault-inducing uplifts and clean uplifts. The decision tree models help us discover that test code churn can affect the fault-proneness of a patch when its PageRank value is low.

Table \ref{tab:rank_mars} shows the top five metrics ranked by the MARS models. Again, code churn is strongly associated with the fault-proneness of the uplifted patches in Aurora and Beta channels. In the Release channel, another code complexity metric, \ie{} the maximum nesting is strongly associated with the fault-proneness of uplifted patches.
%Prior work~\cite{} has also found that high nesting level of loop in a program can increase the debugging and review difficult, even lead post-release faults to users. (I didn't find a good reference)
In general, the most top metrics yielded by the MARS models are code complexity related, which is another reminder to reviewers and release managers that they should carefully inspect complex patches before delivering a positive uplift decision. Reviewers and release managers should also pay close attention to patches submitted by experienced developers, with a large number of words in comments. A recommendation in line with the findings of \textbf{RQ2}. %(accresults of \textbf{RQ2}).

\textbf{Overall, both decision tree and MARS models suggest that release managers should pay close attention to complex patches. Mozilla and other software organizations interested in patch uplifts, should make special rules for reviewing complex patches that are submitted for uplift. If possible, complex patches uplift candidates should be assigned a low priority.} %, since they are more risky than other uplift patch candidates.}


